EPO: Explicit Policy Optimization for Strategic Reasoning in LLMs via Reinforcement Learning

Large Language Models (LLMs) have shown impressive reasoning capabilities in well-defined problems with clear solutions, such as mathematics and coding. However, they still struggle with complex real-world scenarios like business negotiations, which require strategic reasoning-an ability to navigate dynamic environments and align long-term goals amidst uncertainty. Existing methods for strategic reasoning face challenges in adaptability, scalability, and transferring strategies to new contexts. To address these issues, we propose explicit policy optimization (EPO) for strategic reasoning, featuring an LLM that provides strategies in open-ended action space and can be plugged into arbitrary LLM agents to motivate goal-directed behavior. To improve adaptability and policy transferability, we train the strategic reasoning model via multi-turn reinforcement learning (RL),utilizing process rewards and iterative self-play. Experiments across social and physical domains demonstrate EPO's ability of long-term goal alignment through enhanced strategic reasoning, achieving state-of-the-art performance on social dialogue and web navigation tasks. Our findings reveal various collaborative reasoning mechanisms emergent in EPO and its effectiveness in generating novel strategies, underscoring its potential for strategic reasoning in real-world applications. Code and data are available at https://github.com/AlibabaResearch/DAMO-ConvAI/tree/main/EPO.

==> backup.tex <==
% \begin{table*}[ht]
%     \centering
%     \begin{tabular}{llccccc}
%     \toprule
%      \multirow{2}{*}{Backbone} & \multirow{2}{*}{Method}  &  \multicolumn{2}{c}{\textbf{SOTOPIA}} & \multirow{2}{*}{\textbf{WebShop}} & \multicolumn{2}{c}{\textbf{ALFWorld}}\\
%      & & Hard & All &  & Seen & Unseen\\
%      \midrule
%      Llama3-8B & SFT & 6.65 & 8.20 & 62.6 & \textbf{61.4}& \textbf{60.4} \\
%      Llama3-8B & EPO-SFT & \textbf{6.76} & \textbf{8.28} & \textbf{67.1} & 45.9 & 44.1 \\
%      \bottomrule
%     \end{tabular}
%     \caption{\textbf{Comparative performance between training a single LLM with SFT and explicitly optimizing a strategic reasoning model via SFT.}
%     The evaluation metric for SOTOPIA is the final goal completion score, and average reward for WebShop and ALFWorld. Our strategic reasoning model trained with SFT is plugged into GPT-4o.}
%     \label{tab:single_res}
% \end{table*}


% \section{Additional Results}
% \label{append:add_res}

% To validate the effectivess of explicit policy optimization for strategic reasoning, we conduct comparative experiments which involve fine-tuning a single LLM (Llama3-8B-Instruct) via SFT on training data collected from three environments, respectively. This single model is trained to output strategy and behavior simuteneously for each interaction turn. The results are shown in Table~\ref{tab:single_res}.

% From the results, it can be observed that training a single LLM via SFT underperforms our reasoning model trained with SFT plugged into LLM agents (GPT-4o) for navigating in SOTOPIA and WebShop, despite that the LLM agents remain frozen without additional training. However, our method underperforms the single model fined-tuned on ALFWorld, since the frozen LLM agent (GPT-4o) has poor performance in this environment. Under the guidance of our reasoning model in \textit{EPO}, this agent improves performance in achieving long-term goals but still struggles with challenging scenarios in ALFWorld.

==> format-backup.tex <==
\begin{abstract}
This document is a supplement to the general instructions for *ACL authors. It contains instructions for using the \LaTeX{} style files for ACL conferences.
The document itself conforms to its own specifications, and is therefore an example of what your manuscript should look like.
These instructions should be used both for papers submitted for review and for final versions of accepted papers.
\end{abstract}

\section{Introduction}

These instructions are for authors submitting papers to *ACL conferences using \LaTeX. They are not self-contained. All authors must follow the general instructions for *ACL proceedings,\footnote{\url{http://acl-org.github.io/ACLPUB/formatting.html}} and this document contains additional instructions for the \LaTeX{} style files.

The templates include the \LaTeX{} source of this document (\texttt{acl\_latex.tex}),
the \LaTeX{} style file used to format it (\texttt{acl.sty}),
an ACL bibliography style (\texttt{acl\_natbib.bst}),
an example bibliography (\texttt{custom.bib}),
and the bibliography for the ACL Anthology (\texttt{anthology.bib}).

\section{Engines}

To produce a PDF file, pdf\LaTeX{} is strongly recommended (over original \LaTeX{} plus dvips+ps2pdf or dvipdf). Xe\LaTeX{} also produces PDF files, and is especially suitable for text in non-Latin scripts.

\section{Preamble}

The first line of the file must be
\begin{quote}
\begin{verbatim}
\documentclass[11pt]{article}
\end{verbatim}
\end{quote}

To load the style file in the review version:
\begin{quote}
\begin{verbatim}
\usepackage[review]{acl}
\end{verbatim}
\end{quote}
For the final version, omit the \verb|review| option:
\begin{quote}
\begin{verbatim}
\usepackage{acl}
\end{verbatim}
\end{quote}

To use Times Roman, put the following in the preamble:
\begin{quote}
\begin{verbatim}
\usepackage{times}
\end{verbatim}
\end{quote}
(Alternatives like txfonts or newtx are also acceptable.)

Please see the \LaTeX{} source of this document for comments on other packages that may be useful.

Set the title and author using \verb|\title| and \verb|\author|. Within the author list, format multiple authors using \verb|\and| and \verb|\And| and \verb|\AND|; please see the \LaTeX{} source for examples.

By default, the box containing the title and author names is set to the minimum of 5 cm. If you need more space, include the following in the preamble:
\begin{quote}
\begin{verbatim}
\setlength\titlebox{<dim>}
\end{verbatim}
\end{quote}
where \verb|<dim>| is replaced with a length. Do not set this length smaller than 5 cm.

\section{Document Body}

\subsection{Footnotes}

Footnotes are inserted with the \verb|\footnote| command.\footnote{This is a footnote.}

\subsection{Tables and figures}

See Table~\ref{tab:accents} for an example of a table and its caption.
\textbf{Do not override the default caption sizes.}

\begin{table}
  \centering
  \begin{tabular}{lc}
    \hline
    \textbf{Command} & \textbf{Output} \\
    \hline
    \verb|{\"a}|     & {\"a}           \\
    \verb|{\^e}|     & {\^e}           \\
    \verb|{\`i}|     & {\`i}           \\
    \verb|{\.I}|     & {\.I}           \\
    \verb|{\o}|      & {\o}            \\
    \verb|{\'u}|     & {\'u}           \\
    \verb|{\aa}|     & {\aa}           \\\hline
  \end{tabular}
  \begin{tabular}{lc}
    \hline
    \textbf{Command} & \textbf{Output} \\
    \hline
    \verb|{\c c}|    & {\c c}          \\
    \verb|{\u g}|    & {\u g}          \\
    \verb|{\l}|      & {\l}            \\
    \verb|{\~n}|     & {\~n}           \\
    \verb|{\H o}|    & {\H o}          \\
    \verb|{\v r}|    & {\v r}          \\
    \verb|{\ss}|     & {\ss}           \\
    \hline
  \end{tabular}
  \caption{Example commands for accented characters, to be used in, \emph{e.g.}, Bib\TeX{} entries.}
  \label{tab:accents}
\end{table}

As much as possible, fonts in figures should conform
to the document fonts. See Figure~\ref{fig:experiments} for an example of a figure and its caption.

Using the \verb|graphicx| package graphics files can be included within figure
environment at an appropriate point within the text.
The \verb|graphicx| package supports various optional arguments to control the
appearance of the figure.
You must include it explicitly in the \LaTeX{} preamble (after the
\verb|\documentclass| declaration and before \verb|\begin{document}|) using
\verb|\usepackage{graphicx}|.

\begin{figure}[t]
  \includegraphics[width=\columnwidth]{example-image-golden}
  \caption{A figure with a caption that runs for more than one line.
    Example image is usually available through the \texttt{mwe} package
    without even mentioning it in the preamble.}
  \label{fig:experiments}
\end{figure}

\begin{figure*}[t]
  \includegraphics[width=0.48\linewidth]{example-image-a} \hfill
  \includegraphics[width=0.48\linewidth]{example-image-b}
  \caption {A minimal working example to demonstrate how to place
    two images side-by-side.}
\end{figure*}

\subsection{Hyperlinks}

Users of older versions of \LaTeX{} may encounter the following error during compilation:
\begin{quote}
\verb|\pdfendlink| ended up in different nesting level than \verb|\pdfstartlink|.
\end{quote}
This happens when pdf\LaTeX{} is used and a citation splits across a page boundary. The best way to fix this is to upgrade \LaTeX{} to 2018-12-01 or later.

\subsection{Citations}

\begin{table*}
  \centering
  \begin{tabular}{lll}
    \hline
    \textbf{Output}           & \textbf{natbib command} & \textbf{ACL only command} \\
    \hline
    \citep{Gusfield:97}       & \verb|\citep|           &                           \\
    \citealp{Gusfield:97}     & \verb|\citealp|         &                           \\
    \citet{Gusfield:97}       & \verb|\citet|           &                           \\
    \citeyearpar{Gusfield:97} & \verb|\citeyearpar|     &                           \\
    \citeposs{Gusfield:97}    &                         & \verb|\citeposs|          \\
    \hline
  \end{tabular}
  \caption{\label{citation-guide}
    Citation commands supported by the style file.
    The style is based on the natbib package and supports all natbib citation commands.
    It also supports commands defined in previous ACL style files for compatibility.
  }
\end{table*}

Table~\ref{citation-guide} shows the syntax supported by the style files.
We encourage you to use the natbib styles.
You can use the command \verb|\citet| (cite in text) to get ``author (year)'' citations, like this citation to a paper by \citet{Gusfield:97}.
You can use the command \verb|\citep| (cite in parentheses) to get ``(author, year)'' citations \citep{Gusfield:97}.
You can use the command \verb|\citealp| (alternative cite without parentheses) to get ``author, year'' citations, which is useful for using citations within parentheses (e.g. \citealp{Gusfield:97}).

A possessive citation can be made with the command \verb|\citeposs|.
This is not a standard natbib command, so it is generally not compatible
with other style files.

\subsection{References}

\nocite{Ando2005,andrew2007scalable,rasooli-tetrault-2015}

The \LaTeX{} and Bib\TeX{} style files provided roughly follow the American Psychological Association format.
If your own bib file is named \texttt{custom.bib}, then placing the following before any appendices in your \LaTeX{} file will generate the references section for you:
\begin{quote}
\begin{verbatim}
\bibliography{custom}
\end{verbatim}
\end{quote}

You can obtain the complete ACL Anthology as a Bib\TeX{} file from \url{https://aclweb.org/anthology/anthology.bib.gz}.
To include both the Anthology and your own .bib file, use the following instead of the above.
\begin{quote}
\begin{verbatim}
\bibliography{anthology,custom}
\end{verbatim}
\end{quote}

Please see Section~\ref{sec:bibtex} for information on preparing Bib\TeX{} files.

\subsection{Equations}

An example equation is shown below:
\begin{equation}
  \label{eq:example}
  A = \pi r^2
\end{equation}

Labels for equation numbers, sections, subsections, figures and tables
are all defined with the \verb|\label{label}| command and cross references
to them are made with the \verb|\ref{label}| command.

This an example cross-reference to Equation~\ref{eq:example}.

\subsection{Appendices}

Use \verb|\appendix| before any appendix section to switch the section numbering over to letters. See Appendix~\ref{sec:appendix} for an example.

\section{Bib\TeX{} Files}
\label{sec:bibtex}

Unicode cannot be used in Bib\TeX{} entries, and some ways of typing special characters can disrupt Bib\TeX's alphabetization. The recommended way of typing special characters is shown in Table~\ref{tab:accents}.

Please ensure that Bib\TeX{} records contain DOIs or URLs when possible, and for all the ACL materials that you reference.
Use the \verb|doi| field for DOIs and the \verb|url| field for URLs.
If a Bib\TeX{} entry has a URL or DOI field, the paper title in the references section will appear as a hyperlink to the paper, using the hyperref \LaTeX{} package.

\section*{Acknowledgments}

This document has been adapted
by Steven Bethard, Ryan Cotterell and Rui Yan
from the instructions for earlier ACL and NAACL proceedings, including those for
ACL 2019 by Douwe Kiela and Ivan Vuli\'{c},
NAACL 2019 by Stephanie Lukin and Alla Roskovskaya,
ACL 2018 by Shay Cohen, Kevin Gimpel, and Wei Lu,
NAACL 2018 by Margaret Mitchell and Stephanie Lukin,
Bib\TeX{} suggestions for (NA)ACL 2017/2018 from Jason Eisner,
ACL 2017 by Dan Gildea and Min-Yen Kan,
NAACL 2017 by Margaret Mitchell,
ACL 2012 by Maggie Li and Michael White,
ACL 2010 by Jing-Shin Chang and Philipp Koehn,
ACL 2008 by Johanna D. Moore, Simone Teufel, James Allan, and Sadaoki Furui,
ACL 2005 by Hwee Tou Ng and Kemal Oflazer,
ACL 2002 by Eugene Charniak and Dekang Lin,
and earlier ACL and EACL formats written by several people, including
John Chen, Henry S. Thompson and Donald Walker.
Additional elements were taken from the formatting instructions of the \emph{International Joint Conference on Artificial Intelligence} and the \emph{Conference on Computer Vision and Pattern Recognition}.

==> rebuttal/general-response.tex <==
We greatly appreciate the insightful and high-quality comments from all reviewers. We are particularly encouraged that reviewers recognize the generalization capability, scalability, strategy transparency, transferability and simplicity of our proposed method as well as its potential for real-world applications.

We have addressed all questions of reviewers in each individual response. According to the suggestions of reviewers, we also conduct a series of additional experiments and include the results and discussions in the revised paper. Below is a summary of paper updates and new experiments.
\begin{itemize}
    \item 
SFT
RL
EPO-SFT
EPO-SFT+RL
\end{itemize}

We hope that the updated results and our responses have addressed the concerns reviewers have. We will release our reasoning models, RL data and code once published. Please let us know if there are any other questions or suggestions.





==> rebuttal/rebuttal-1.tex <==
\textbf{Q1:} A more detailed comparison using policy optimization with SFT is needed to strengthen the argument that the multi-turn RL pipeline eliminates the need for SFT as a preliminary step.

\textbf{A1:}
SFT
EPO-SFT
EPO-SFT+RL w/PRM


\textbf{Q2:} The computation costs of training the reasoning model through RL.

\textbf{A2:}
4 A100 GPU, training time 40 mins, llama3-8B
similar to SFT
high computational efficiency and policy optimization. 




\textbf{Q3:} Failure case discussion of EPO.

\textbf{A3:}
select one failture case from sotopia (e.g., low goal completion)


\textbf{Q4:} Why is EPO-Llama3-8B w/RL better on unseen ALFWorld with Llama3-8B-Instruct than on seen task types?

\textbf{A4:} 
similar performance. (14.3 vs. 14.5). check 14.3 and 14.5. 用条数解释（对了多少）


We will add a societal impact section to discuss the safeguards of the strategic reasoning model.




==> rebuttal/rebuttal-2.tex <==
\textbf{Q1:} The process evaluation metrics depend heavily on GPT-4o, introducing potential bias and reproducibility issues.

\textbf{A1:}

2. why we choose GPT-4o as the PRM.
3. how to address potential bias: a simple binary classification task; GPT-4o for evaluation, llama3-8B or GPT-turbo as the model for generating strategy data for process evaluation. but any model even human annotators may introduce bias during process evaluation.
4. how to address reproducibility: llama-3-70B as PRM
1. Without PRM, the RL is still better than EPO-SFT. show results.


\textbf{Q2:} Additional experiment based on llama3-8B for PPDPP.

\textbf{A2:}
1. why we maintain roberta-large for PPDPP. encoder for classification. predicted strategies: five action types
2. llama3-8B: decoder for text generation. predicted strategies: open-ended strategy in natural language form. require other modifications, such as ####. not a fair comparison. 
test qwen-0.5B (roberta-large:0.37B)

==> rebuttal/rebuttal-3.tex <==
\textbf{Q1-The choice of evaluation benchmark:} The value of using WebShop and ALFWorld as evaluation datasets and test on other strategic reasoning tasks. 

\textbf{A1:}
1. Why we choose WebShop and ALFWorld as evaluation benchmarks for strategic reasoning.

To stress-test the efficacy of EPO, we need environments and task setups that satisfy several
desiderata. First, the chosen tasks must require strategic multi-step planning and reasoning under
delayed rewards, and cannot be solved in one turn. We also want these tasks to require LLMs to
generate coherent natural language and keep the task realistics.
These tasks require strategic reasoning and planning over long horizons, allow non-trivial success rates, and come equipped with reproducible and task-directed evaluation metrics.~\cite{pmlr-v235-zhou24t}.

WebShop and ALFWorld are two physical domains in contrast to Sotopia which is a social domain, to further demonstrate the generalization of our method across different domains, which is a challenging issue to LLM reasoning~\cite{patil2025advancing}.


Thought: a rationale/short-CoT as the strategy
For example,



2. sotopia already contains some negotiation games as in Game-theoretic LLM, such as Prisoner's Dilemma (a complete-information game) and Deal/No Deal (an incomplete-information game).
Show corresponding results (goal and overall score and dialogues).
hightlight the challenge of sotopia.

3. the text games (such as Guess my city and twenty questions) in Archer are simpler and less realistic compared to Sotopia. As you mentioned, WebShop is also tested in Archer to evaluate model's strategic multi-step planning and reasoning under sparse rewards (see Section 5.1 in~\cite{pmlr-v235-zhou24t}).



\textbf{Q2-Evaluation performance:} SFT does even better than EPO-SFT on ALFWorld, and small gains in Tables 1 and 2, particularly in Sotopia.

\textbf{A2:}
We have illustrated the possible reason in line 1024-1025 in Appendix E.

goal completion [0-10] in line 378.
overall score [-4.286, 5.714] averaged across seven evaluation dimensions (as illustrated in Appendix B-\textbf{SOTOPIA}.

\begin{table*}[h]
    \centering
    \begin{tabular}{c|c}
    \toprule
      Dimension   &  Range \\
      \midrule
      Goal   & [0, 10]\\
      Believability & [0, 10]\\
      Knowledge & [0, 10]\\
      Relationship & [-5, 5] \\
      Finantial & [-5, 5]\\
      Secret & [-10, 0]\\
      Social rules & [-10, 0]\\
      \bottomrule
    \end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table*}



\textbf{Q3-Comparison with other RL baselines:} Most of the comparisons that take place are with prompting based methods, and directly treating the agent as a policy and training with REINFORCE would be simple to compare to.

\textbf{A3:}
1. baselines are not mostly prompting-based methods (only Vanilla and ReAct are prompting-based methods).
PPDPP and DAT are not.
Additional baselines: variants of EPO are not. three variants of EPO-RL
(1) EPO-Llama3-8B w/SFT has already achieved comparable or superior performance compared to EPO-GPT-4o (results). 
(2) EPO-Llama3-8B w/RL further surpasses EPO-llama3-8B w/SFT even in the setting without the use of PRM ().
(3) Using PRM and iterative self-play further boosts the performance of EPO-Llama3-8B w/RL ().

2. Llama3-8B RL 
EPO-Llama3-8B-RL w/o PRM
EPO-Llama3-8B-RL w/ PRM
EPO-Llama3-8B-RL w/ PRM + Self-play


\textbf{Q4-Supports for the second claim in contributions:}  Improvement in policy transferability and a cost comparison between EPO +RL+Self-Play and methods that use SFT as a preliminary step.

\textbf{A4:}
1. experimental settings to validate the policy transferability: Training scenarios and evaluation scenarios are completely non-overlapping. Show scenarios particularly from SOTOPIA-hard (evaluation) that are unseen during training (SOTOPIA-$\pi$).
different instructions in WebShop test scenarios and training ones.
Unseen evaluation scenarios in ALFWorld. 

2.  SFT as a preliminary step: SFT initialized model for RL.
results and training costs comparison
EPO-SFT+RL 
EPO-RL w/ PRM + Self-play (见的数据量是一样的）






